SN 2020sck: deflagration in a carbon-oxygen white dwarf

We present optical UBVRI photometry and low-to-medium resolution spectroscopic observations of type Iax SN 2020sck spanning -5.5 d to +67 d from maximum light in the B-band. From the photometric analysis we find $\Delta m_{\rm{B}}$(15) = 2.03$\pm$0.05 mag and $M_{\rm{B}}$=-17.81$\pm$0.22 mag. Radiation diffusion model fit to the quasi-bolometric light curve indicates 0.13$\pm$0.02 $M_{\odot}$ of $^{56}$Ni and 0.34 $M_{\rm \odot}$ of ejecta are synthesized in the explosion. Comparing the observed quasi-bolometric light curve with angle-averaged bolometric light curve of three-dimensional pure deflagration explosion of $M_{\rm{ch}}$ carbon-oxygen white dwarf, we find agreement with a model in which 0.16 $M_{\odot}$ of $^{56}$Ni and 0.37 $M_{\odot}$ of ejecta is formed. By comparing the +1.4 day spectrum of SN 2020sck with synthetic spectrum generated using SYN++, we find absorption features due to C II, C III and O I. These are unburned materials in the explosion and indicate a C-O white dwarf. One dimensional radiative transfer modeling of the spectra with TARDIS shows higher density in the ejecta near the photosphere and a steep decrease in the outer layers with an ejecta composition dominated mostly by C, O, Si, Fe, and Ni. The star formation rate of the host galaxy computed from the luminosity of the H$\alpha$ ($\lambda$6563) line is 0.09 $M_{\odot}$ yr$^{-1}$ indicating a relatively young stellar environment.

==> Tables/typeIax_sample.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{10pt}
\caption{Properties of the comparison sample.}
\label{tab:SNIax_sample}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c c c c c c}
\hline
SN   &   Distance Modulus  &    Extinction       &  $M_{\rm B}$     &  $M_{\rm V}$  &  $\Delta m_{\rm 15}(B)$  & $\Delta m_{\rm 15}(g)$ &  12 + log($\rm \frac{O}{H}$) &  Reference \\
(Name)     &       (mag)         &      $E(B-V)$ (mag) &   (mag)      & (mag)     & (mag)   & (mag)       & (dex)    &       \\
\hline\hline  
SN~2002cx &  35.09$\,\pm\,$0.32 &  0.034         &   -17.53$\,\pm\,$0.26    &  -17.49$\,\pm\,$0.22  & 1.70$\,\pm\,$0.1  & -- & --  & 1, 2 \\
SN~2005hk &  33.46              &  0.110         &   -18.02$\,\pm\,$0.32    &  -18.08$\,\pm\,$0.29  & 1.68$\,\pm\,$0.05 & 1.36$\,\pm\,$0.01 & --  & 2, 3 \\
SN~2008ha &  31.64              &  0.081         &   -13.74$\,\pm\,$0.15    &  -14.21$\,\pm\,$0.15  & 2.17$\,\pm\,$0.02  & 1.80$\,\pm\,$0.03 &8.16$\,\pm\,$0.15  & 4 \\
SN~2009ku &  --                 &   --           &           --             &   -18.4               & 0.59               & --  & 5  \\
SN~2010ae &  30.58$\,\pm\,$0.58 &  0.62$\,\pm\,$0.42 & -13.44$\,\pm\,$0.54  &   -13.80              & 2.43$\,\pm\,$0.11  & 1.51$\,\pm\,$0.05 & 8.40$\,\pm\,$0.18  & 6  \\
SN~2011ay &  34.69$\,\pm\,$0.17 &  0.081         &    -18.15$\,\pm\,$0.17   &   -18.39$\,\pm\,$0.18 & 1.11$\,\pm\,$0.16  & --  & 7 \\
SN~2012Z  &  32.4$\,\pm\,$0.30  &  0.036         &    -17.61                &   -18.04              & 1.57$\,\pm\,$0.07  & 1.30$\,\pm\,$0.01 &8.51$\,\pm\,$0.31   & 8 \\
PS1-12bwh &  34.91$\,\pm\,$0.15 &  0.26$\,\pm\,$0.07 & --                   &   --                  & --                 & 1.35$\,\pm\,$0.09 & 8.87$\,\pm\,$0.19   & 9 \\
SN~2013en &  34.11$\,\pm\,$0.15 &  0.500         &     --                   &    --                 & --                 & -- & --  & 10 \\ 
SN~2014ck &  31.94$\,\pm\,$0.15 &  0.50$\,\pm\,$0.10 & -17.37$\,\pm\,$0.15  &   -17.29$\,\pm\,$0.15 & 1.76$\,\pm\,$0.15  & 1.59$\,\pm\,$0.1 & --  & 11 \\  
SN~2014dt &  31.66$\,\pm\,$0.01 &  0.02          &     -18.13$\,\pm\,$0.04  &   -18.33$\,\pm\,$0.02 & 1.35$\,\pm\,$0.06  & -- & --  & 12  \\
SN~2014ek &  34.99$\,\pm\,$0.20 &  0.054         &     -17.32$\,\pm\,$0.23  &   -17.66$\,\pm\,$0.20 & 1.54$\,\pm\,$0.17  & -- & --  & 13  \\
SN~2015H  &  33.91$\,\pm\,$0.07 &  0.048         &     --                   &    --                 & --                 & -- & --  & 14 \\
SN~2019gsc & 33.60              &  0.08          &     --                   &    --                 & --                 & -- & 8.10$\,\pm\,$0.06  & 15 \\
SN~2019muj & 32.66$\,\pm\,$0.18 & 0.023          &     -16.36$\,\pm\,$0.06  &   -16.42$\,\pm\,$0.0  & 2.4 & 2.0 &   --  & 16 \\
\hline
%\multicolumn{6}{l}{\rlap{*}\  ~in unit of mag (100 d)$^{-1}$ and epoch is relative to $B$ band maximum.}
\end{tabular}}
\newline \newline
References:\
(1) \citet{2003PASP..115..453L}; (2) \citet{2007PASP..119..360P} (3) \citet{2008ApJ...680..580S}; (4) \citet{2009AJ....138..376F}; (5) \citet{2011ApJ...731L..11N}; (6) \citet{2014A&A...561A.146S}; (7) \citet{2015MNRAS.453.2103S}; (8) \citet{2015ApJ...806..191Y}; 
(9) \citet{2017A&A...601A..62M}; (10) \citet{2015MNRAS.452..838L}; (11) \citet{2016MNRAS.459.1018T}; (12) \citet{2018MNRAS.474.2551S}; (13) \citet{2018MNRAS.478.4575L}; (14) \citet{2016A&A...589A..89M}; (15) \citet{2020ApJ...892L..24S}; (16) \citet{2021MNRAS.501.1078B}
\end{table*}
%\end{rotatetable}
